Identification and validation of the dynamic model of a tendon-driven anthropomorphic finger

This study addresses the absence of an identification framework to quantify a comprehensive dynamic model of human and anthropomorphic tendon-driven fingers, which is necessary to investigate the physiological properties of human fingers and improve the control of robotic hands. First, a generalized dynamic model was formulated, which takes into account the inherent properties of such a mechanical system. This includes rigid-body dynamics, coupling matrix, joint viscoelasticity, and tendon friction. Then, we propose a methodology comprising a series of experiments, for step-wise identification and validation of this dynamic model. Moreover, an experimental setup was designed and constructed that features actuation modules and peripheral sensors to facilitate the identification process. To verify the proposed methodology, a 3D-printed robotic finger based on the index finger design of the Dexmart hand was developed, and the proposed experiments were executed to identify and validate its dynamic model. This study could be extended to explore the identification of cadaver hands, aiming for a consistent dataset from a single cadaver specimen to improve the development of musculoskeletal hand models.

==> _notation.tex <==


% m       joint dimension
% n       tendon dimension   

% M, N, G  rigid body dynamics
% h       joint viscoelasticity
% C       coupling matrix
% ft      tendon force
% ff      tendon friction
% fext    external force

% J       Jacobian




Color:
Tendon 
    1 (PIP): blue
    2 (Extensor): purple
    3 (abduction): red
    4 (adduction): black







==> todo.tex <==
PIN
junnan li
lingyun chen: 296908
Ringwald : 220371
Edmundo: 210169
Amartya: 223070
Sami: 108317
#################

revision:
Dexmart writting in Finger design








Background:
1. Few studies focus on the modelling and parameter identification of a tendon-driven finger/hand for control and manipulation.  

2. There is still no consistent dataset of cadaver hand that contains major aspects of the physiological properties, i.e. moment arm curves, passive properties of joints, and fingertip forces. 

3. The validation scenarios of the biomechanical human hand model are mainly static; and few for robotic hand models. 

Contribution:
1. generalized dynamic model of tendon-driven finger

2. proposing an identification approach for stepwise identifying and validating the parameters of dynamic finger model. 
3. validating the identification approach on several robotic fingers using modular finger design and hand testbed. 

Future work: 
1. comparing the performance of the model-based and model-free control of grasping 

2. proposing the entire workflow, including:

    a. modular finger design 
    
    b. identification testbed for general tendon-driven system 
    
    c. modelling and identification approach
    
    d. model-based control and manipulation
    
    e. feedback on the finger design


% Introduction
% Literature review: 
%     dynamic model of robotic finger/hand
%     musculoskeletal hand model 
%     identification setup 
%     identification method
%     application of the model in control 



% Method
% modelling: 
%     model of the exemplary finger
%     tension distribution algorithms
%     data processing 
%     forward/inverse simulation

% testbed:
%     sensor calibration
%     support frame
%     tendon controller 
%     data acquisition

% identification:
%     optimization method 

% validation
%     comparison of motion or torque?

% modular finger design
    % awiwi finger 
    % dexmarkt finger
    % hand group finger






% limitation:
    % haven't been validated in cadaver study
    % do not model the extensor mechanism of the human finger 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

1. R. King, “Development and validation of a bond graph tendon model of the human finger with the anatomically correct testbed (ACT) hand,” Ph.D. dissertation, University of Utah, Salt Lake City, UT, 2015.

The study proposed a dynamic bond graph model of the finger tendon system. 
The model was validated on ACT hand but showed significant error due to the joint static friction.


2. Tigue, J. A., & Mascaro, S. A. (2017). VALIDATION OF FINGERTIP FORCE AND FINGER POSE IN THE UART FINGER AND BOND GRAPH TENDON MODEL DURING SURFACE CONTACT. Dynamic Systems and Control Conference, 1–8.

Therefore, Utah University developed a new testbed called UART to mitigate static joint friction such that the prediction of the joint position and fingertip force in quasi-static conditions is improved. 
They emphasized that the validation scenario of the fingertip interacting with the force sensor should be an impedance process instead of rigid contact by fixing the fingertip on the sensor.

The joint stiffness is neglected in their model since the rotary spring is not implemented in the testbed; however, this property is critical in the biological human hand system. 


3. Tigue, J. A., & Mascaro, S. A. (2019). Calibration and validation of dynamic model for simulating robotic finger kinematics and contact forces. Dynamic Systems and Control Conference 2019, 1–10.

This study applied several experiments to identify the parameters of a dynamic bond graph model for the anthropomorphic UART finger and proposed an advanced validation scenario that simulates the dynamic interaction force of the fingertip. However, the passive joint stiffness is not included in the model due to the lack of corresponding mechanics in the UART finger, which is indicated as a critical property of the human finger.


4. Deshpande, A. D., Balasubramanian, R., Ko, J., & Matsuoka, Y. (2010). Acquiring variable moment arms for index finger using a robotic testbed. IEEE Transactions on Biomedical Engineering, 57(8), 2034–2044. https://doi.org/10.1109/TBME.2010.2048326


This study proposed a methodology for measuring and calculating the configuration-dependent moment arm of ACT index finger using a Gaussian Processes approach. 
